Prosody-Driven Privacy-Preserving Dementia Detection

Speaker embeddings extracted from voice recordings have been proven valuable for dementia detection. However, by their nature, these embeddings contain identifiable information which raises privacy concerns. In this work, we aim to anonymize embeddings while preserving the diagnostic utility for dementia detection. Previous studies rely on adversarial learning and models trained on the target attribute and struggle in limited-resource settings. We propose a novel approach that leverages domain knowledge to disentangle prosody features relevant to dementia from speaker embeddings without relying on a dementia classifier. Our experiments show the effectiveness of our approach in preserving speaker privacy (speaker recognition F1-score .01%) while maintaining high dementia detection score F1-score of 74% on the ADReSS dataset. Our results are also on par with a more constrained classifier-dependent system on ADReSSo (.01% and .66%), and have no impact on synthesized speech naturalness.

==> sections/introduction_archive.tex <==
\section{Introduction}
\label{sec:intro}

Advances in deep learning, combined with non-invasive biomarkers like speech, offer a promising opportunity for large-scale disease diagnosis. Researchers have investigated the use of speech signals for detecting different medical conditions, such as neurodegenerative diseases (e.g., Parkinson’s and Alzheimer’s)~\cite{de2020cross} and respiratory ailments (e.g., COVID-19)~\cite{ casanova2021transfer}.
%pompili2017automatic, sleep apnea and botelho2019speech,

Speaker embeddings (e.g., i-vector, x-vector, and ECAPA-TDNN) are a type of feature set utilized in the detection of early signs of diseases like dementia~\cite{botelho2022challenges}.
%, jin2023consen, 9747167, pompili2020inesc,, zargarbashi2019multi, heo2022separating
These embeddings contain speaker-specific information, which is crucial in various downstream tasks such as automatic speaker verification (ASV), speaker diarization, zero-shot text-to-speech (TTS), and voice cloning. However, they often contain more information than required for their intended tasks, which poses potential privacy concerns. This unintentional information leakage might violate GDPR policies~\cite{gdpr} and its data minimization principle~\cite{gdprSensitiveData} (i.e., ``adequate, relevant and limited to what is necessary in relation to the purposes for which they are processed''), leaving individuals vulnerable to discrimination, extortion, and targeted advertisements by third parties.
%qian2019autovc
In this paper, we discuss how to use prosody disentanglement as a method for obscuring attributes in dementia detection. Specifically, we aim to maintain the dementia attribute in speaker embeddings while reducing speaker-related information (identity). Often, adversarial training or multi-task learning is utilized to confine information within bottlenecks, separating out dimensions such as content, pitch, rhythm, and timbre~\cite{qian2020unsupervised}. However, we take a different approach, focusing on prosodic features that are known to be prominent in dementia speech, such as articulation rate, pauses, and disfluencies. Our hypothesis is that by disentangling these features from speaker representations, we can effectively obscure the speaker's identity while minimizing any impact on dementia-related information. Our system achieves this without relying on dedicated classifiers, using domain knowledge and adversarial learning techniques.

%Dementia, a neurodegenerative disease characterized by cognitive decline, can be detected from speaker embeddings. Previous studies have leveraged speaker embeddings as acoustic representations for automatic dementia detection using i-vectors and x-vectors~\cite{jin2023consen, 9747167, pompili2020inesc, heo2022separating, zargarbashi2019multi}. However, 
%this information leakage is not intended and goes against the General Data Protection Regulation (GDPR)~\cite{gdpr} policies and its data minimization principle~\cite{gdprSensitiveData} which emphasises that personal data should be ``adequate, relevant and limited to what is necessary in relation to the purposes for which they are processed''. Consequently, this privacy issue can leave individuals vulnerable to discrimination, extortion, and targeted advertisements by financial institutions and employers.

%The General Data Protection Regulation (GDPR)~\cite{gdpr} policies consider speech data and its representations as biometric data, and therefore, sensitive personal data. Particularly, the GDPR's principles of privacy-by-design and data protection, particularly Article 25~\cite{gdprSensitiveData}, emphasises the data minimisation principle whereby personal data should be “adequate, relevant and limited to what is necessary in relation to the purposes for which they are processed”. The information leakage goes against this principle and can lead to discrimination, extortion, and targeted advertisements by financial institutions and employers.

%Author et al.~\cite{} have demonstrated that by removing speaker information from the embeddings they improve dementia detection, highlighting the importance of content and paralinguistic cues embedded within these representations.

%Attributes obfuscation, prosody disentanglement is often achieved with adversarial training or multi-task learning. To do this, carefully crafted bottlenecks to constrain information could be implemented~\cite{qian2020unsupervised, qian2019autovc} to perform disentangling transformations on the data itself to isolate dimensions such as content, pitch, rhythm and timbre. In this paper, we investigate prosody disentanglement as a means to obfuscate dementia-related information in speaker embeddings, free of a dementia discriminator. Previous studies investigated acoustic features relevant to dementia speech and found prosodic features such as articulation rate, pauses and disfluencies to be the most prominent characteristics. We hypothesize that isolating those features from speaker representations can help obfuscate Dementia while having minimal impact on the speaker's information. To this end, we implement a system using domain knowledge that leverages adversarial learning to disentangle prosody features key to dementia, without the need for a dementia classifier. 

%Additionally, work like SpeechSplit\cite{qian2020unsupervised} and AutoVC~\cite{qian2019autovc} uses carefully crafted bottlenecks to constrain information. SpeechSplit2~\cite{chan2022speechsplit2} 

The~\textbf{main contributions} of this paper are
\begin{enumerate}
\item \textbf{Novel Approach}: We propose a novel method for preserving privacy in speaker embeddings for low-resource settings through domain knowledge and prosody disentanglement.
\item \textbf{Privacy Preservation without Dedicated Classifiers}: Unlike previous methods that rely on dedicated classifiers, our system achieves privacy preservation without the need for attribute-specific classifiers. 
\item \textbf{New application Domain} We shed light on a new and sensitive attribute, dementia, that has not been extensively investigated in previous attribute obfuscation and anonymization works.
\end{enumerate}


==> sections/related_work.tex <==
\section{Speaker Anonymity \& Disentanglement}

Anonymization or de-identification refers to the task of concealing the speaker’s identity while retaining the linguistic content, thereby making the data unlinkable~\cite{tomashenko2020introducing}. According to the ISO/IEC International Standard 24745 on biometric information protection~\cite{ISO/IEC}, biometric references must be irreversible and unlinkable for full privacy protection. Most of the proposed
works focus on protecting/anonymizing speaker identity using
voice conversion (VC) mechanisms~\cite{ srivastava2020evaluating}, however, they are ineffective when the attacker has complete knowledge of the VC scheme and target speaker mapping~\cite{srivastava2020evaluating}.
%peri2023study,noe2020adversarial,
Attribute-driven privacy preservation involves allowing a speaker to conceal specific personal aspects in their voice representation while still maintaining overall performance~\cite{aloufi2020privacypreserving, noe2022bridge}. Beyond speaker
identity, various works propose to protect speakers's attributes and paralinguistic information such as emotion~\cite{aloufi2019emotionless,chouchane2023differentially, noe2022bridge,teixeira2023privacy}, age~\cite{ teixeira2023privacy} or nationality~\cite{luu2022investigating}. 
%zargarbashi2019multi, stoidis2022generating, heo2022separating, luu2022investigating
Adversarial training disentangles dimensions in latent spaces for speaker verification while minimizing detection of specific attributes~\cite{chouchane2023differentially}. However, the need of an external attribute classifier is a considerable limitation, particularly for low-resource attributes with no training data, especially in the case of medical conditions such as dementia. An alternative approach to anonymizing speech is to work at the feature level rather than the utterance level~\cite{noe2022bridge, lavania2023utility, tran23b_interspeech}. By extracting and sanitizing feature representations from speech utterances, we can release privacy-aware features instead of full speech utterances. These features, obtained from pre-trained encoders, serve various downstream tasks effectively. Noé et. al., in~\cite{noe2022bridge}, for example, proposed a non-linear discriminant analysis using a Normalizing Flow-based architecture to disentangle sex information from speaker identity in a x-vector neural embeddings. 

%Prosodic features are often studied in voice conversion and speech synthesis, where they are selected and isolated based on the specific task. 
%Attribute-driven privacy preservation as the idea of enabling a speaker to hide only a few personal aspects in its voice representation while maintaining the remaining particularities and the performance of a desired task~\cite{}. Several recent works have delved into the study of obfuscating speaker attributes and paralinguistic information such as emotion~\cite{aloufi2019emotionless,chouchane2023differentially,noe2020adversarial,noe2022bridge,teixeira2023privacy,zargarbashi2019multi,peri2023study, stoidis2022generating,heo2022separating}, age~\cite{luu2022investigating,peri2023study,teixeira2023privacy} or nationality~\cite{luu2022investigating} within speech. These approaches utilize adversarial training to disentangle dimensions in latent spaces. For example,  enabling speaker verification while avoiding the detection of a specific speaker attribute. They use an adversarial autoencoding approach that disentangles and hides a given binary attribute (i.e., sex) in a x-vector neural embedding. This method is based on an encoder-decoder architecture combined with an additional classifier that tries to predict the attribute class from the encoded representation. However, while these studies on voice anonymisation and demographic-level attributes, there remains a gap in addressing medical health conditions such as Alzheimer's disease.

%Hiding information within speech has been mostly studied in the light of anonymization, the task of removing a speaker's identity within a sample. Several recent works have delved into the study of obfuscating speaker attributes and paralinguistic information such as emotion~\cite{aloufi2019emotionless,chouchane2023differentially,noe2020adversarial,noe2022bridge,teixeira2023privacy,zargarbashi2019multi,peri2023study, stoidis2022generating,heo2022separating}, age~\cite{luu2022investigating,peri2023study,teixeira2023privacy} or nationality~\cite{luu2022investigating} within speech. These approaches utilize adversarial training to disentangle dimensions in latent spaces. Noé et. al.,~\cite{noe2020adversarial} have employed an autoencoder with pre-trained classifiers to remove gender information. Luu et. al.,~\cite{luu2022investigating} have combined multi-task and adversarial learning to disentangle speaker identity. Peri et al. have added dimensionality reduction and mutual information loss to remove gender and age information. Lavania et. al.,~\cite{lavania2023utility} have detected emotion-related features using a pre-trained emotion classifier. Lastly, Chouchane et. al.,~\cite{chouchane2023differentially} have isolated sex-related information using an adversarially trained gender classifier and differentially private noise. However, while these studies on voice anonymisation and demographic-level attributes, there remains a gap in addressing medical health conditions such as Alzheimer's disease.

%However, several recent work have investigated obfuscating speaker attributes and paralinguistic information such as gender~\cite{aloufi2019emotionless,chouchane2023differentially,noe2020adversarial,noe2022bridge,teixeira2023privacy,zargarbashi2019multi,peri2023study, stoidis2022generating,heo2022separating}, age~\cite{luu2022investigating,peri2023study,teixeira2023privacy} or nationality~\cite{luu2022investigating}. Most approaches leverage adversarial training to disentangle specific dimensions within the latent space. In the realm of speaker representations, Noé et al.~\cite{noe2020adversarial}, implement an autoencoder with an external pre-trained classifier and a gender classifier trained on the latent space to remove gender information.

%Luu et al.~\cite{luu2022investigating} combine multi-task learning and adversarial learning to disentangle speaker identity from gender, age and nationality, into two latent spaces. They observe that the gender dimension has a significant impact the ASV accuracy. In a work by Peri et al., ~\cite{peri2023study}, they add a dimensionality reduction step and mutual information loss on top of the adversarial loss to remove gender and age information. In Lavania et al.~\cite{lavania2023utility} they find that adversarial learning is not sufficient to remove speaker information while preserving emotion classification. Instead, they detect the most important features of emotion detection within the latent representations, using a pre-trained emotion classifier, and shuffle the remainder. Chouchane et al.~\cite{chouchane2023differentially} uses an adversarially trained gender classifier to isolate sex-related information in the encoded latent space and apply differentially private noise. Introducing a control mechanism to quantify gender-specific privacy. In Texeira et al.~\cite{teixeira2023privacy}, the method proposed in this paper consists of a combination of a Vector Quantized Variational AutoEncoder (VQ-VAE), trained to reconstruct the true speaker embedding, an adversarial attribute classifier for age and gender and a non-parametric Mutual Information (MI) estimator as a loss function. In ~\cite{stoidis2022generating}, they generate gender-ambiguous voices using a GAN model conditioned on the ground truth gender label. Nevertheless, the need for an external attribute classifier is a considerable limitation in the case of low-resource attributes with no training data and does not guarantee generalisation to other classifiers. In the case of medical conditions such as dementia, publicly available datasets are scarce. Recently, Noé et al.~\cite{noe2022bridge}. proposed a non-linear discriminant analysis based on a Normalising Flow-based architecture to disentangle sex information from the speaker identity within a latent representation. 







==> sections/temp.tex <==


\begin{table}[htbp]
    \centering
    \caption{Comparison of anonymization systems' performance. The table shows the dementia detection f1-score (AD), speaker recognition f1-score (SPK), and equal error rate (EER) for each system.}
    \label{tab:overall_res}
   \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{System} & \textbf{AD} & \textbf{SPK} & \textbf{EER (\%)} \\
        \midrule
        Original & .81 & .33 & 35 \\
        \midrule
        ADV SPK$_{AD}$ + AD & .64 & .00 & 47 \\
        ADV SPK$_{LibriSpeech}$ & .85 & .68 & 15 \\
        ADV PROS & .75 & .00 & 43 \\
        \midrule
        Shuffle$_{Random}$ & .64  & .02  & 41  \\
        Shuffle$_{Shap}$ & .63 & .02 & 41 \\
        Shuffle$_{MI\_AD}$ & .65  & .02  & 41  \\
        Shuffle$_{MI\_pros}$ & .65 & .02 & 44 \\
        \bottomrule
    \end{tabular}%
    }
\end{table}




\begin{table}[htbp]
    \centering
    \caption{Comparison of anonymization systems' performance. The table shows the dementia detection f1-score (AD), speaker recognition f1-score (SPK), and equal error rate (EER) for each system.}
    \label{tab:overall_res}
   \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{System} & \textbf{AD} & \textbf{SPK} & \textbf{EER (\%)} \\
        \midrule
        Original & .81 & .33 & 35 \\
        \midrule
        ADV SPK$_{AD}$ + AD & .64 & .00 & 47 \\
        ADV SPK$_{LibriSpeech}$ & .85 & .68 & 15 \\
        ADV PROS & .75 & .00 & 43 \\
        \midrule
        Shuffle$_{Random}$ & .64  & .02  & 41  \\
        Shuffle$_{Shap}$ & .63 & .02 & 41 \\
        Shuffle$_{MI\_AD}$ & .65  & .02  & 41  \\
        Shuffle$_{MI\_pros}$ & .65 & .02 & 44 \\
        \bottomrule
    \end{tabular}%
    }
\end{table}
